Decomposing Disease Descriptions for Enhanced Pathology Detection: A Multi-Aspect Vision-Language Pre-training Framework

Medical vision language pre-training (VLP) has emerged as a frontier of research, enabling zero-shot pathological recognition by comparing the query image with the textual descriptions for each disease. Due to the complex semantics of biomedical texts, current methods struggle to align medical images with key pathological findings in unstructured reports. This leads to the misalignment with the target disease's textual representation. In this paper, we introduce a novel VLP framework designed to dissect disease descriptions into their fundamental aspects, leveraging prior knowledge about the visual manifestations of pathologies. This is achieved by consulting a large language model and medical experts. Integrating a Transformer module, our approach aligns an input image with the diverse elements of a disease, generating aspect-centric image representations. By consolidating the matches from each aspect, we improve the compatibility between an image and its associated disease. Additionally, capitalizing on the aspect-oriented representations, we present a dual-head Transformer tailored to process known and unknown diseases, optimizing the comprehensive detection efficacy. Conducting experiments on seven downstream datasets, ours improves the accuracy of recent methods by up to 8.56% and 17.26% for seen and unseen categories, respectively. Our code is released at https://github.com/HieuPhan33/MAVL.

==> tab/aspects.tex <==
{\footnotesize\begin{table*}[t]
\centering
\caption{List of generated aspects of MIMIC's medical findings after experts' curations.}
\label{tab:gen}
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Normal & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and smooth, with the edge of the lung tissue appearing as a thin, curved line against the ribs.
\item Fluid: no fluid or effusion accumulation.
\item Location: fills the chest cavity, from just below the collarbones to just above the diaphragm.
\item Opacity: balanced, neither too opaque (white) nor too transparent (dark).
\item Other: symmetric appearance between two chest's sides; clear visibility of the heart, ribs, spine, and diaphragm; bronchial tubes and blood vessels are visible as white lines or tree-branch patterns against the darker lung tissue.
\item Patterns: no cloudy or patchy areas, no concentrated white or black spots.
\item Shape: lungs appear as two large, oval or triangular areas on either side of the heart.
\item Texture: uniform with small, branching white lines representing the bronchi and blood vessels.
\end{itemize}\\
\midrule
Clear & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, sharp borders of the heart, lungs, and diaphragm.
\item Fluid: no fluid or effusion accumulation.
\item Location: no abnormal shadows or spots in any part of the lung.
\item Opacity: normal transparency, neither too white nor too dark.
\item Other: symmetric appearance between two chest's sides; diaphragm and costophrenic angles are clearly visible; no abnormal growths or masses.
\item Patterns: visible bronchial tree and vascular markings without any cloudiness.
\item Shape: regular, well-defined shapes of the heart, lungs, and diaphragm.
\item Texture: uniform, with no patchy or cloudy areas.
\end{itemize}\\
\midrule
Sharp & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, with a distinct separation from surrounding tissues.
\item Fluid: no fluid or effusion accumulation.
\item Location: predictable based on the anatomical structure being viewed. for instance, ribs will be located on either side of the chest.
\item Opacity: structures such as bones appear very bright or white on the x-ray due to their high density.
\item Other: bones and other dense structures will stand out clearly against the darker, less dense lung tissue.
\item Patterns: regular and symmetrical, following the natural pattern of the anatomical structure. for example, ribs will appear in parallel lines.
\item Shape: sharp, well-defined shapes that follow the natural structure of the anatomical part, like the clear outline of a rib or the spine.
\item Texture: smooth and uniform, without the patchy or speckled appearance seen in lung tissue.
\end{itemize}\\
\midrule
Sharply & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, sharp, and distinct, not blending into the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: varies, depending on the part of the lung or chest being examined.
\item Opacity: normal, balanced transparency and opacity, neither too white nor too dark.
\item Other: symmetric appearance between two chest's sides; clear lung fields; visible and defined structures such as ribs, heart, and major blood vessels.
\item Patterns: regular and consistent, not patchy or irregular.
\item Shape: clear, defined edges and shape, not fuzzy or blurred.
\item Texture: smooth, regular, and consistent texture.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel1}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Effusion & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, sharp border along the top of the effusion.
\item Fluid: fluid accumulation is the main feature, which causes a cloudy appearance.
\item Location: typically located at the base of the lungs, between the lung and chest wall.
\item Opacity: more opaque, appearing whiter or cloudier than the surrounding lung tissue.
\item Other: possible displacement of other structures such as the heart or trachea; reduction in lung volume; and increased density at the base of the lung.
\item Patterns: no specific patterns, effusion spreads out in the pleural space.
\item Shape: typically appears as a meniscus, or curved shape, at the lung base.
\item Texture: smooth texture, without any grainy or mottled appearance.
\end{itemize}\\
\midrule
Pleural Opacity & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: borders may be well-defined or blurry, depending on the underlying cause of the opacity.
\item Fluid: opacities can be caused by fluid accumulation, inflammation, infection, or a mass.
\item Location: can be in any part of the lung.
\item Opacity: appears as a white or light gray area on the x-ray, which is denser than the surrounding tissue.
\item Other: may cause a change in the appearance or position of nearby structures, such as the heart, blood vessels, or airways.
\item Patterns: may have a patchy or uniform appearance.
\item Shape: can vary, but usually is irregular or round.
\item Texture: usually appears solid, without a specific texture.
\end{itemize}\\
\midrule
Pneumothorax & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: well-defined and sharp, often following the contour of the rib cage.
\item Fluid: no fluid accumulation, the space is filled with air.
\item Location: typically seen at the periphery of the lung, often toward the upper part.
\item Opacity: less opaque and more transparent, often appearing darker than the surrounding lung tissue.
\item Other: possible shift of the heart and mediastinum to the opposite side; visible pleural line; and reduced lung volume on the affected side.
\item Patterns: absence of normal lung markings beyond the line of the collapsed lung, giving a 'black' or 'empty' appearance.
\item Shape: a clear, distinct line indicating the edge of the lung, which has collapsed or become compressed.
\item Texture: smooth, devoid of the usual markings seen in lung tissue.
\end{itemize}\\
\midrule
Edema & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: fuzzy or blurred, gradually blending into the surrounding lung tissue.
\item Fluid: fluid accumulation or effusion with cloudy appearance.
\item Location: usually affects both lungs and often located at the lung's base.
\item Opacity: more opaque, and less transparent, appearing like a cloudy or hazy spot.
\item Other: increased vascular markings, increased heart size, and increased lung volume.
\item Patterns: uniform density with a \"bat-wing\" or \"butterfly\" pattern.
\item Shape: typically spreads out irregularly, not in a clear, defined shape.
\item Texture: fine, grainy, or mottled texture within the cloudy area, looking like small, speckled spots.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel3}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Atelectasis & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear or sharp border if there is a total collapse, blurry if partial.
\item Fluid: fluid accumulation or effusion may be present if atelectasis is due to a blockage.
\item Location: can be anywhere in the lung, but often near the middle.
\item Opacity: more opaque, and less transparent, appearing as a dense or white area.
\item Other: the diaphragm, heart, and trachea may shift towards the affected side; the affected lung may appear smaller; ribs may be closer together on the affected side.
\item Patterns: no specific patterns. the collapsed area is generally uniform in appearance.
\item Shape: can be irregular depending on the part of the lung that has collapsed.
\item Texture: denser, more solid-looking texture in the collapsed area.
\end{itemize}\\
\midrule
Tube & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, distinctly separate from the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: depending on its purpose, it could be in the trachea (breathing tube), in the chest cavity (chest tube), or inserted into a blood vessel (central line).
\item Opacity: can be very opaque, appearing white against the darker lung tissue.
\item Other: metal markers may be present; can be seen entering or exiting the body; may be connected to outside equipment.
\item Patterns: no specific patterns, it appears as a straight line or curve.
\item Shape: generally straight and cylindrical, like a straw or tube.
\item Texture: smooth with no grainy or mottled texture.
\end{itemize}\\
\midrule
Consolidation & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: margins are often indistinct, blending into the surrounding lung tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: can occur anywhere in the lung but often seen in lower lobes.
\item Opacity: more opaque, and less transparent, often appearing whiter or cloudier.
\item Other: possible shift in mediastinum (central organs) towards the affected side if volume loss is present, asymmetric appearance between the two sides of the chest.
\item Patterns: no specific patterns, but can show an 'air bronchogram' – dark, branching structures within the white, dense area.
\item Shape: irregular, dense patches which may be round, oval, or lobe-shaped.
\item Texture: smooth or homogeneous texture within the affected area.
\end{itemize}\\
% \midrule
% Process & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
% \item Border: the borders of the lungs may appear clearer or fuzzier, depending on the process.
% \item Fluid: presence of fluid in or around the lungs, which would appear as darker, shadowy areas.
% \item Location: any abnormalities might be localized to a specific area of the lung or distributed throughout.
% \item Opacity: depending on the process, there could be areas that are more opaque (whiter) or less opaque (darker).
% \item Other: changes in the size or position of the heart, shifts in the mediastinum, or presence of foreign bodies.
% \item Patterns: changes in normal patterns, such as the appearance of spots, streaks, or lines that were not previously present.
% \item Shape: irregular or regular shapes in the lung that are not typically there.
% \item Texture: changes in the texture of the lung tissue, it could be coarse, rough, or grainy.
% \end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel4}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Abnormality & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: irregular or indistinct, not clearly defined against the surrounding area.
\item Fluid: unexpected fluid accumulation or effusion with a cloudy appearance.
\item Location: any area of the lung where it does not match its counterpart on the other side.
\item Opacity: unusual whiteness or darkness compared to surrounding lung tissue.
\item Other: asymmetry between the two sides of the chest; unexpected objects or shadows; changes in the size or shape of the heart or major blood vessels; or changes in the position of the diaphragm or mediastinum.
\item Patterns: unusual patterns or clusters of opacity that do not follow regular lung structures.
\item Shape: unexpected or irregular shapes in areas where lung tissue should be.
\item Texture: unusual texture, either too smooth or too uneven compared to normal lung tissue.
\end{itemize}\\
\midrule
Enlarge & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear but expanded, extending beyond the normal boundary of the heart.
\item Fluid: no specific fluid accumulation related to the heart enlargement.
\item Location: centered in the chest, between the two lungs.
\item Opacity: more opaque and less transparent, appearing whiter than the surrounding tissue.
\item Other: widening of the mediastinum (the space between the lungs where the heart is located); displacement of the bronchi, trachea or esophagus; and compressing or pushing the lungs to either side.
\item Patterns: the enlarged heart will look like a silhouette, its shape clearly outlined against the lighter lung tissue.
\item Shape: the heart will appear larger and broader than normal, often taking up more than half of the chest's width.
\item Texture: dense and solid, similar to the surrounding lung tissue.
\end{itemize}\\
\midrule
Tip & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, distinctly separating it from the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be located anywhere in the chest, depending on the type of tip.
\item Opacity: more opaque and less transparent, appearing as a small, bright and dense spot.
\item Other: metallic appearance, can be seen as a small, bright, and dense spot against the lung's dark background.
\item Patterns: no specific patterns, usually a single, isolated spot.
\item Shape: usually round or oval, similar to the tip of a needle or a pin.
\item Texture: smooth and uniform, without any changes or irregularities.
\end{itemize}\\
\midrule
Low & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the borders of the lungs may appear closer to the center of the chest.
\item Fluid: no fluid or effusion accumulation.
\item Location: entire lung region.
\item Opacity: normal or less opaque, depending on the cause of the low lung volume.
\item Other: flattened diaphragm, narrowed intercostal spaces, the ribs may appear closer together, and the chest may appear smaller.
\item Patterns: no specific patterns, but the lung fields may appear condensed.
\item Shape: the heart and mediastinum may appear larger due to the reduced size of the lungs.
\item Texture: normal texture in the lung area.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel5}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Unremarkable & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp borders of the lungs, heart, and diaphragm.
\item Fluid: no fluid or effusion accumulation, no cloudy appearance.
\item Location: heart and lungs are positioned normally, and the diaphragm is at the right level.
\item Opacity: normal and even, neither too white nor too dark.
\item Other: symmetric appearance between two chest's sides; normal size and positioning of the heart; clearly visible bronchial tubes and blood vessels; no signs of abnormalities or disease.
\item Patterns: even distribution of lung markings, no patches or spots.
\item Shape: clear and regular outline of the heart, lungs, and bones.
\item Texture: uniform and smooth texture of the lungs, indicating normal air-filled spaces.
\end{itemize}\\
\midrule
Intact & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and distinct borders of lungs, heart, and bones.
\item Fluid: no fluid or effusion accumulation.
\item Location: lungs, heart, and bones are in their correct positions.
\item Opacity: well-balanced opacity, not too white or too dark.
\item Other: symmetric appearance between two chest's sides; clear rib cage; normal heart size; normal lung volume.
\item Patterns: evenly spread vascular markings, no abnormal clusters or patches.
\item Shape: regular, symmetrical shape of lungs and heart.
\item Texture: smooth, even texture with no abnormal spots or patches.
\end{itemize}\\
\midrule
Stable & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and well-defined borders of the lungs, heart, and diaphragm.
\item Fluid: no fluid or effusion accumulation.
\item Location: all organs and structures in their expected locations.
\item Opacity: normal transparency, neither too opaque nor too clear.
\item Other: symmetric appearance between two chest's sides; no irregular or unusual dark or light areas.
\item Patterns: no unusual or abnormal patterns.
\item Shape: normal shape of lungs, heart, bones, and other structures.
\item Texture: smooth, even texture with no unusual spots or patches.
\end{itemize}\\
\midrule
Free & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: sharp, clear, and distinct line separating the air from other tissues.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be found in various locations, but often seen beneath the diaphragm, around the lungs, or in the chest cavity.
\item Opacity: less opaque and more transparent, appearing darker compared to other tissues.
\item Other: asymmetrical appearance between two sides of the chest; visible outline of certain structures like the diaphragm, heart, or lung lobes due to the air outlining these structures.
\item Patterns: no specific pattern, often appears as a darker or empty space.
\item Shape: irregular or uneven in shape.
\item Texture: smooth, without any texture or pattern, similar to an empty space.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel2}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Pneumonia & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: fuzzy or unclear, blending into the surrounding lung tissue.
\item Fluid: fluid accumulation or effusion with cloudy appearance.
\item Location: vary in different parts of the lung.
\item Opacity: more opaque and less transparent, appearing whiter or cloudier than the surrounding lung tissue.
\item Other: asymmetric appearance between two chest's sides, cloudiness near the lung's edges, dark lines standing out against the cloudy background.
\item Patterns: cloudy areas that are not evenly spread and have a clustered or patchy appearance.
\item Shape:  irregular, patchy areas in the lung.
\item Texture: fluffy or grainy texture within the lung area, similar to a snowy tv screen.
\end{itemize}\\
\midrule
Line & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and well-defined, unlike the fuzzy or unclear borders of some other findings.
\item Fluid: no fluid or effusion accumulation along the line.
\item Location: can be anywhere, but often seen running vertically or horizontally across the lung field.
\item Opacity: may vary from opaque to slightly transparent, depending on the material of the line.
\item Other: lines can be tubes, wires, or other foreign objects; they stand out against the lung tissue and bones as they are often more opaque.
\item Patterns: lines typically don't have a pattern per se, but multiple lines may cross or intersect.
\item Shape: straight or curved, but always elongated and narrow.
\item Texture: smooth and consistent along the length of the line.
\end{itemize}\\
\midrule
Congestion & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: borders are not clear, blending into the surrounding tissue.
\item Fluid: possible fluid accumulation or effusion with a cloudy appearance.
\item Location: often affects both lungs and often located in the lower parts of the lungs.
\item Opacity: increased opacity, appearing as a whiter or less transparent area.
\item Other: increased lung volume, increased vascular markings, and possible signs of heart enlargement.
\item Patterns: non-uniform, patchy distribution of opacity.
\item Shape: irregular, not clearly delineated.
\item Texture: grainy, uneven, or mottled texture within the lung area.
\end{itemize}\\
\midrule
Catheter & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, distinct from the surrounding tissue.
\item Fluid: no fluid or effusion accumulation along the catheter line.
\item Location: depending on the type of catheter, it may be seen entering the body at various points and extending into specific organs or vessels. for example, a central venous catheter often enters at the neck or chest and extends towards the heart.
\item Opacity: catheter appears very bright or white in comparison to the surrounding tissues.
\item Other: may have associated hardware, such as ports or discs, visible.
\item Patterns: straight or slightly curved line, depending on the path the catheter takes through the body.
\item Shape: long, thin, tube-like structure.
\item Texture: smooth and consistent, with no grainy or patchy appearance.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel6}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Cardiomegaly & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the borders of the heart may appear rounded or bulging outwards.
\item Fluid: there may be fluid accumulation around the heart or in the lungs.
\item Location: the heart is located centrally in the chest.
\item Opacity: the heart area appears more opaque and less transparent, appearing as a large, white, central mass.
\item Other: the silhouette of the heart may occupy more than half of the chest's width, making the mediastinum appear wider. the blood vessels may also appear enlarged.
\item Patterns: no specific patterns, but the overall size and shape of the heart is larger and rounder than normal.
\item Shape: the heart appears larger than normal, often extending beyond the normal boundaries.
\item Texture: the texture of the heart doesn't change, but the shape and size are what indicate cardiomegaly.
\end{itemize}\\
\midrule
Fracture & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the edges of the fracture are typically sharp and irregular.
\item Fluid: there may be surrounding soft tissue swelling but no fluid or effusion accumulation within the bone.
\item Location: can occur in any part of the chest, including the ribs or collarbone.
\item Opacity: the fracture area will often appear whiter or more opaque than the surrounding tissue.
\item Other: there may be multiple fractures; the bone ends may overlap or be driven into each other; there may be changes in the alignment of the bone structures.
\item Patterns: the fractured bone may be displaced or move out of its normal alignment.
\item Shape: an abnormal, irregular line or break in the continuity of the bone.
\item Texture: the area around the fracture may be jagged, rough, or splintered.
\end{itemize}\\
\midrule
Air & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear or sharp, especially if air is trapped within a normally solid structure like lung tissue.
\item Fluid: absence of fluid or effusion accumulation.
\item Location: can be in various parts of the chest, including the lungs, pleural space, or mediastinum.
\item Opacity: less opaque or more transparent, often appearing darker or even black.
\item Other: asymmetric appearance between two chest's sides; dark area; contrast between air-filled spaces and surrounding tissues; hollow, tubular structures in the lung can appear more prominent if filled with air.
\item Patterns: no specific patterns, typically appearing as clear, dark areas on the x-ray.
\item Shape: no specific shape, as air can fill different structures in the chest.
\item Texture: smooth, consistent, and homogenous area without speckles or spots.
\end{itemize}\\
\midrule
Tortuous & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and distinct, following the path of the blood vessel.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be anywhere in the lung where blood vessels are present.
\item Opacity: normal or slightly less opaque, the focus is on blood vessels rather than lung tissue.
\item Other: blood vessels may appear larger or thicker; there might be a gradual change in the vessel's direction.
\item Patterns: the vessel follows a winding or irregular path, rather than a direct or straight one.
\item Shape: blood vessels appear twisted or coiled, not following a straight line.
\item Texture: clear and smooth, as it is the vessel's route that is of interest.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel7}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Lead & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, sharp, and distinct.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be anywhere, depending on where the lead entered the body.
\item Opacity: more opaque and less transparent, appearing as bright white spots or lines.
\item Other: metallic density; may appear as isolated spots or lines; asymmetry between the two sides of the chest; lead objects can cast a shadow or appear brighter than bones.
\item Patterns: no specific patterns, though lead pellets may cluster together.
\item Shape: typically round or oval if it's a pellet, or long and thin if it's a line.
\item Texture: smooth, consistent, and dense.
\end{itemize}\\
\midrule
Disease & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the edges of the lungs and other structures may be blurred or sharp, depending on the disease. for example, in emphysema, the borders of the lungs may be less distinct due to the breakdown of lung tissue.
\item Fluid: if there is fluid in or around the lungs, it can indicate disease. for instance, pleural effusion, which is excess fluid between the layers of the pleura, can be seen in conditions like pneumonia or heart failure.
\item Location: some diseases may affect specific parts of the lungs. for instance, tuberculosis often affects the upper lobes of the lungs.
\item Opacity: depending on the disease, some areas of the lungs may appear more opaque (whiter) or less opaque (darker) than normal lung tissue.
\item Other: additional signs of disease
\item Patterns: certain diseases can cause specific patterns on the x-ray. for instance, a 'honeycomb' pattern may indicate interstitial lung disease.
\item Shape: the shape of the lungs and other structures in the chest may be altered. for example, tumors may appear as round, oval, or irregularly shaped masses in the lungs.
\item Texture: changes in texture can also indicate disease. for example, fibrosis can cause a coarse, irregular texture in the lung tissue.
\end{itemize}\\
\midrule
Calcification & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: well-defined, sharp, and clear, making the calcified area stand out.
\item Fluid: typically, no fluid or effusion accumulation.
\item Location: can occur anywhere in the lungs, but often seen near the heart or major blood vessels.
\item Opacity: more opaque, appearing brighter or whiter than surrounding tissues.
\item Other: may be associated with other signs of lung disease or damage, such as fibrosis or scarring.
\item Patterns: scattered or clustered depending on the cause.
\item Shape: can vary, but often appears as small, round or irregularly shaped spots.
\item Texture: dense, hard texture that stands out against softer lung tissue.
\end{itemize}\\
\midrule
Prominence & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and well-defined, highlighting the prominence of the structure.
\item Fluid: no fluid or effusion accumulation.
\item Location: depends on the prominent structure. for example, if a blood vessel is prominent, it will appear in the lung fields; if the heart is prominent, it will appear in the center of the chest.
\item Opacity: normal or slightly enhanced, not as white as pneumonia or as dark as pneumothorax.
\item Other: the structure appears larger or more noticeable than usual, such as prominent blood vessels, a large heart, or bulging ribs.
\item Patterns: no specific patterns, but the structure is more noticeable.
\item Shape: the shape of the structure is more noticeable or larger than usual.
\item Texture: normal texture, but the structure appears more pronounced or swollen.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel8}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Device & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, as metals have a high density that creates a clear contrast with the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: depends on the device. endotracheal tubes are in the trachea, chest tubes are in the chest wall, pacemakers are in the chest close to the heart, stents are in the blood vessels.
\item Opacity: typically metallic and very bright white, standing out against the surrounding tissue.
\item Other: wires or tubes can be seen extending from the device, connecting it to the outside of the body or to other organs. devices might also be attached to the bones or the heart.
\item Patterns: linear for tubes, box-like for devices like pacemakers, circular or elliptical for stents.
\item Shape: depends on the device. tubes are long and linear, pacemakers are small and box-like, stents are cylindrical.
\item Texture: smooth, with uniform density.
\end{itemize}\\
\midrule
Engorgement & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the borders of the blood vessels will be clearer and more pronounced.
\item Fluid: no fluid or effusion accumulation.
\item Location: typically seen in the blood vessels of the heart and lungs.
\item Opacity: more opaque, appearing denser or whiter compared to surrounding areas.
\item Other: enlarged heart, prominent pulmonary artery, and increased lung volume.
\item Patterns: blood vessels may appear more prominent or crowded, particularly around the heart.
\item Shape: no specific shape, but the blood vessels of the lung and heart appear larger.
\item Texture: the blood vessels will appear as thicker, denser lines.
\end{itemize}\\
\midrule
Inserted central catheter & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, as the catheter is a solid object.
\item Fluid: no fluid or effusion accumulation related to the catheter.
\item Location: inserted in the upper arm and travels towards the large vein above the heart.
\item Opacity: the catheter appears as a bright, distinct, white line.
\item Other: may be coiled or kinked in some situations; the catheter's tip should ideally be located at the junction of the superior vena cava and the right atrium in the heart.
\item Patterns: follows the route of the veins, seen as a white line within the darker vein.
\item Shape: linear and long, extending from the insertion site towards the heart.
\item Texture: smooth and consistent, different from the surrounding tissue.
\end{itemize}\\
\midrule
Clip & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, distinctly different from the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be found anywhere, but usually seen in the lung or heart area if it's a surgical clip.
\item Opacity: very opaque or bright white, standing out against the surrounding tissue.
\item Other: may cast a shadow or appear as a foreign object on the x-ray.
\item Patterns: no specific patterns, as it is an artificial object.
\item Shape: often small, rectangular or round, depending on its type.
\item Texture: smooth and solid, with no texture similar to lung tissue.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel9}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Elevation & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: normal or clear borders of lung tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: displaced structures, like diaphragm or heart, shifted upwards.
\item Opacity: normal or unchanged opacity.
\item Other: increased space below the diaphragm; the heart may appear elongated or stretched; structures like the stomach, liver, or spleen may be pushed down.
\item Patterns: normal lung patterns, but structures present in abnormal positions.
\item Shape: displacement or shifting of structures, such as the diaphragm or the heart.
\item Texture: normal or unchanged texture of the lung tissue.
\end{itemize}\\
\midrule
Expand & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and well-defined, but may seem stretched or expanded.
\item Fluid: no fluid or effusion accumulation.
\item Location: entire lung area, but especially noticeable near the edges.
\item Opacity: less opaque and more transparent, appearing darker.
\item Other: increased lung volume, ribs may appear more spaced out, diaphragm may appear flattened due to the lung's expansion.
\item Patterns: normal lung patterns, but with the overall lung area appearing larger.
\item Shape: lungs appearing larger or inflated.
\item Texture: normal lung texture, but with possibly more air spaces visible.
\end{itemize}\\
\midrule
Nodule & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: well-defined edges that clearly separate it from the surrounding lung tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be found anywhere in the lung.
\item Opacity: more opaque or whiter than surrounding lung tissue.
\item Other: size typically less than 3 cm in diameter, uniform in density, can have a hollow or "cavitary" appearance.
\item Patterns: solitary, isolated spot that stands out from rest of the lung tissue.
\item Shape: round or oval shape.
\item Texture: dense, with a consistent texture.
\end{itemize}\\
\midrule
Wire & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, sharp, and solid line.
\item Fluid: no fluid or effusion accumulation related to the wire.
\item Location: can be anywhere depending on where the wire is placed.
\item Opacity: appears very bright, often white.
\item Other: stands out against the dark background of lung tissue; it may cross over bones and organs.
\item Patterns: usually follows a regular linear or curved pattern.
\item Shape: straight or curved line depending on the shape of the wire.
\item Texture: smooth and consistent texture.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel10}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Pleural Fluid & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: sharp and well-defined, as fluid collects in confined spaces such as the pleural cavity.
\item Fluid: visible fluid accumulation or effusion, appearing as white or cloudy areas.
\item Location: typically found at the base of the lung or in the pleural cavity, which is the space between the lung and the chest wall.
\item Opacity: more opaque and less transparent, appearing whiter or cloudier.
\item Other: displacement of structures, such as the trachea or heart, away from the fluid. the fluid-filled area can also cause the nearby lung tissue to appear compressed or collapsed.
\item Patterns: fluid levels can appear as horizontal lines, or as a meniscus (curved line) when the fluid is in the pleural cavity.
\item Shape: can vary, but often appears in the shape of a crescent or a horizontal line at the base of the lung.
\item Texture: smooth and homogeneous, similar to a body of water on a calm day.
\end{itemize}\\
\midrule
Degenerative & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: may become blurred or irregular in areas of bone loss or destruction.
\item Fluid: typically does not involve fluid accumulation.
\item Location: can occur in any bone or joint, but common locations include the spine, hips, and knees.
\item Opacity: variable, can appear more opaque in areas of calcification or bone spur formation.
\item Other: asymmetry between sides; bone spurs or outgrowths; changes in the shape or alignment of bones or joints; and reduced joint space in areas of cartilage loss.
\item Patterns: no specific patterns, but may see areas of increased density in areas of calcification or bone growth.
\item Shape: may show irregular or altered shapes of bones or joints.
\item Texture: varies, can have a rough or uneven appearance, particularly in areas of joint space narrowing.
\end{itemize}\\
\midrule
Pacemaker & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, distinct from the surrounding tissue.
\item Fluid: no fluid or effusion accumulation.
\item Location: typically located in the upper left or right chest, just below the collarbone. the leads are visible as thin, bright lines extending into the heart.
\item Opacity: visible metallic object, brighter and more opaque than the surrounding tissue.
\item Other: wires (leads) are visible from pacemaker to the heart; the device may be seen under the skin; no lung tissue or bone abnormality associated with it.
\item Patterns: no specific pattern, but the device and leads are distinct and visible.
\item Shape: rectangular or rounded, depending on the type of pacemaker.
\item Texture: smooth, solid, and shiny appearance.
\end{itemize}\\
\midrule
Thicken & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: sharp or blurry, depending on the stage and severity of the condition.
\item Fluid: absence or presence of fluid can vary, depending on the underlying condition.
\item Location: can occur anywhere within the chest cavity, including the lungs and heart.
\item Opacity: more opaque and less transparent, often appearing whiter or denser than the surrounding tissue.
\item Other: increased size or mass in the chest, distortion of surrounding structures, or presence of nodules or tumors.
\item Patterns: may present as concentrated areas of increased density or diffuse thickening throughout the lung.
\item Shape: can be linear, irregular, or circular, depending on the underlying condition.
\item Texture: rough or uneven texture, similar to a thick layer of paint.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel11}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Marking & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear but not sharp, as they are usually small and thin.
\item Fluid: no fluid or effusion accumulation.
\item Location: spread throughout the lungs, but more prominent near the heart and major blood vessels.
\item Opacity: usually appears darker against the lighter colored lungs.
\item Other: increased visibility or density of these markings may suggest certain diseases such as pulmonary edema, fibrosis, or chronic bronchitis.
\item Patterns: branching or web-like pattern, often following the paths of the blood vessels.
\item Shape: thin and linear, similar to small branches or tree roots.
\item Texture: smooth, not chunky or patchy like other lung abnormalities.
\end{itemize}\\
\midrule
Scar & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the borders can be clear and sharp if the scar is old or well-defined; however, they can be fuzzy or blurred in the case of a new scar.
\item Fluid: no fluid or effusion accumulation.
\item Location: can be found anywhere in the lung but often near the place of injury or infection.
\item Opacity: scar tissue often appears more opaque and less transparent, showing up as a lighter or whitish area.
\item Other: the size, shape, and appearance of the scar may change over time; may cause distortion or displacement of adjacent structures.
\item Patterns: no specific patterns, scar tissue appears as an isolated lighter patch.
\item Shape: usually a round or irregular patch, it might also appear as a linear or band-like structure.
\item Texture: typically smoother and denser than the surrounding lung tissue.
\end{itemize}\\
\midrule
Hyperinflate & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the border of the lungs may be pushed outwards, towards the rib cage.
\item Fluid: no fluid or effusion accumulation.
\item Location: affects the entire lung area.
\item Opacity: normal or slightly less opaque, with increased transparency.
\item Other: increased lung volume, the heart may appear vertically oriented or elongated, the spaces between the ribs may appear larger than normal.
\item Patterns: more space between the ribs, and the diaphragm may appear flattened.
\item Shape: expanded or enlarged size of the lung fields.
\item Texture: normal or slightly less dense.
\end{itemize}\\
\midrule
Blunt & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: may be sharp if there's a fracture, or blurred if there's a contusion.
\item Fluid: potential fluid accumulation, or hemothorax, if there's internal bleeding.
\item Location: can occur anywhere based on the impact site, often seen in chest wall, ribs, or lung fields.
\item Opacity: varying opacity depending on the injury, may appear more opaque due to damage or accumulated fluid.
\item Other: fractured ribs may appear as sharp, jagged lines. lung contusions could appear as cloudy, opaque areas. the shape of the chest cavity may also change due to the blunt force.
\item Patterns: no specific patterns as it depends on the type and severity of injury.
\item Shape: may show irregular shapes due to fractures or contusions.
\item Texture: could vary, potentially grainy or mottled due to internal damage.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel12}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Loss & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: depending on the type of loss, the border may be clear and sharp or irregular.
\item Fluid: no fluid or effusion accumulation.
\item Location: can occur in various parts of the lung.
\item Opacity: less opaque and more transparent, often appearing darker.
\item Other: asymmetric appearance between two chest's sides; dark area; sharper contrast between the lung and the ribs; reduced lung volume.
\item Patterns: absence of normal lung patterns, like bronchi or vessels.
\item Shape: depending on the type of loss, the shape may be irregular or missing entirely.
\item Texture: smooth, empty, or hollow texture in areas where there should be lung tissue.
\end{itemize}\\
\midrule
Widen & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, as it's usually a structural change and not a lesion or disease.
\item Fluid: no fluid or effusion accumulation.
\item Location: could be anywhere depending on what structure is widened (e.g., widened mediastinum, widened pulmonary artery).
\item Opacity: the area of interest appears more solid and less transparent than the surrounding tissue.
\item Other: a widened structure will often cause a displacement or compression of its neighboring structures. this can cause a change in the shape or position of these structures, making them appear abnormal.
\item Patterns: no specific patterns, but the structure in question will appear larger than normal.
\item Shape: enlargement or expansion in an area that should be narrower.
\item Texture: no specific texture, but rather a dimensional change.
\end{itemize}\\
\midrule
Collapse & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp boundaries, especially if the collapse is complete.
\item Fluid: no fluid or effusion accumulation.
\item Location: can occur in any part of the lung.
\item Opacity: more opaque and less transparent, appearing whiter compared to surrounding lung tissue.
\item Other: possible shift of the heart, trachea, and major bronchi towards the affected side; increased visibility of the ribs and the diaphragm on the side of collapse.
\item Patterns: no specific patterns, but the affected lobe or segment is shrunk in size.
\item Shape: area of collapse may appear as a linear, wedge-shaped, or rounded opacity depending on the extent of collapse.
\item Texture: dense, solid texture in the collapsed area.
\end{itemize}\\
\midrule
Density & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: well-defined borders may suggest denser tissues, while fuzzy or blurred borders can indicate less dense tissues.
\item Fluid: fluid appears denser or whiter than air-filled spaces, but less dense than bone or other solid tissues.
\item Location: high density often appears in bones and heart, while low density typically seen in the lungs.
\item Opacity: the denser the tissue, the whiter or brighter it appears on the x-ray image.
\item Other: dense areas may cast shadows or obscure other structures on the x-ray image.
\item Patterns: abnormal patterns in tissue density can indicate diseases or conditions such as tumors or fibrosis.
\item Shape: irregular or unusual shapes can suggest abnormal tissue density.
\item Texture: texture can vary depending on the type of tissue; for example, bone appears very dense and white, while air-filled lungs appear darker.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel13}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Emphysema & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp lung borders.
\item Fluid: no fluid or effusion accumulation.
\item Location: often spread evenly throughout the lungs, but more pronounced in upper lobes.
\item Opacity: less opaque and more transparent, often appearing darker.
\item Other: flattened diaphragm, increased lung volume, widened spaces between the ribs, and decreased heart size.
\item Patterns: dark areas of the lung, reduced vascular markings.
\item Shape: the lungs may appear larger or over-inflated.
\item Texture: thin, sparse lung tissue, loss of normal markings.
\end{itemize}\\
\midrule
Aerate & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: entire lung field is clear with sharp, defined borders.
\item Fluid: no fluid or effusion accumulation is seen.
\item Location: spreads evenly throughout the lungs.
\item Opacity: normal, balanced opacity, not too white or too dark.
\item Other: symmetric appearance between two chest's sides; clear, defined rib and heart outlines.
\item Patterns: no specific patterns, no patchy or cloudy areas.
\item Shape: lungs appear clear and well-defined with normal contours.
\item Texture: smooth, even texture throughout the lung area.
\end{itemize}\\
\midrule
Mass & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the edges may be well-defined in some cases, but they can also be irregular or spiculated.
\item Fluid: there may be fluid accumulation or pleural effusion in some cases, which appears as an additional layer of opacity on the lung's edge.
\item Location: can occur anywhere in the lung, but often seen near the hilum (the central part of the lung where the bronchi and blood vessels enter).
\item Opacity: typically more opaque and less transparent, appearing as a dense, white or gray mass.
\item Other: enlarged lymph nodes in the mediastinum (the area between the lungs), loss of volume in a part of the lung, or displacement of other structures in the chest.
\item Patterns: single or multiple masses or nodules. the tumor may also cause collapse of the lung or airway obstruction, leading to an area of increased opacity.
\item Shape: irregular, round or oval shape. can also look like a spiculated mass, which means it has spikes or points sticking out.
\item Texture: solid, dense, and uniform texture within the mass.
\end{itemize}\\
\midrule
Crowd & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: borders of the individual bronchovascular structures may become less distinct due to their increased density and crowding.
\item Fluid: no typical fluid or effusion accumulation.
\item Location: typically affects both lungs and can occur in any part of the lung.
\item Opacity: no significant changes in opacity, but closer inspection may show more white or dense areas due to congested vessels.
\item Other: an overall increased density and crowding of the lung structures, often associated with conditions that lead to fluid accumulation or inflammation, such as heart failure or pneumonia.
\item Patterns: no specific patterns, but the overall appearance of the lung fields may be more chaotic or cluttered.
\item Shape: no characteristic shape, but the normal structures of the lung such as the bronchi and vessels may appear more crowded or denser.
\item Texture: texture of the lung field may appear more cluttered or chaotic due to the increased density of the bronchovascular structures.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel14}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Infiltrate & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: fuzzy, unclear, blending into the surrounding lung tissue.
\item Fluid: may or may not have fluid or effusion accumulation, depending on the cause of the infiltrate.
\item Location: can occur in any part of the lung.
\item Opacity: more opaque and less transparent, appearing as a cloudy or hazy area.
\item Other: asymmetric appearance; can be seen as singular or multiple spots, isolated or diffused areas.
\item Patterns: cloudy areas that are not evenly spread and have a patchy or reticular appearance.
\item Shape: irregular, not clearly defined, and tends to blend into surrounding lung tissue.
\item Texture: grainy, patchy, or uneven texture within the cloudy area.
\end{itemize}\\
\midrule
Obscure & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the edges may be unclear or fuzzy, blending into the surrounding lung tissue.
\item Fluid: may or may not show fluid accumulation, depending on the underlying issue.
\item Location: can be anywhere in the lung, depending on where the issue is.
\item Opacity: the affected area will be less transparent, appearing as a cloudy or shaded area.
\item Other: changes in size or shape of lung structures; asymmetry between the two sides of the chest; presence of foreign bodies or masses. note: the term "obscure" isn't specific to a particular disease or finding. it generally means that an area is hard to interpret or understand on the x-ray due to overlapping structures, poor image quality, or a complex underlying issue. therefore, the features can vary widely.
\item Patterns: may show non-uniform or irregular patterns within the affected area.
\item Shape: could be irregular and not well-defined, depending on the underlying issue.
\item Texture: can be different from the surrounding lung tissue, appearing denser or more grainy.
\end{itemize}\\
\midrule
Deformity & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: irregular or unusual borders, not clearly defined or straight.
\item Fluid: no specific fluid accumulation related to deformity itself.
\item Location: can be anywhere in the chest, but often affects the spine or ribs.
\item Opacity: varies depending on the type of deformity. some areas may be more opaque or less transparent.
\item Other: disproportionality between different parts of the chest, misalignment of the spine or ribs, asymmetry between two sides of the chest.
\item Patterns: abnormal patterns, such as twisted or curved lines, or areas of unusual density.
\item Shape: abnormal shape of the chest, spine, ribs, or other parts of the chest. it might appear twisted, curved, or irregular.
\item Texture: varies depending on the type of deformity. some areas may have a different texture than the surrounding tissue.
\end{itemize}\\
\midrule
Hernia & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear, distinct, and well-defined.
\item Fluid: no fluid or effusion accumulation unless the hernia is strangulated, which might show fluid-filled bowel loops.
\item Location: depends on the type of hernia, but commonly near the abdomen or diaphragm.
\item Opacity: can vary, but often appears as a darker, round or oval shape in the chest or abdomen area.
\item Other: displacement of adjacent structures, for instance, pushing the lung tissue away; can also see the presence of bowel loops or fat within the chest.
\item Patterns: usually a single, isolated shape, but can also appear as multiple shapes if there are multiple hernias.
\item Shape: typically round or teardrop-shaped.
\item Texture: it can appear empty or filled, depending on the contents of the hernia.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel15}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Drainage & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, showing the outline of the draining tube.
\item Fluid: fluid accumulation or effusion may be seen near the tube, but it usually decreases over time as the drainage process continues.
\item Location: anywhere within the chest cavity; often seen near the lung's periphery, but can also be central, depending on where the drainage tube is placed.
\item Opacity: variable depending on the drained fluid but generally appears less opaque than the surrounding lung tissue.
\item Other: presence of the radiopaque line of the drainage tube, and possible decrease in size of any previously noted fluid collections or lung opacities.
\item Patterns: no specific patterns, the drainage tube appears as a clear tubular structure.
\item Shape: tubular with a clear defined shape, often showing a hollow interior.
\item Texture: smooth texture within the tube and around it.
\end{itemize}\\
\midrule
Distention & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and sharp, but the structures may appear larger or more pronounced.
\item Fluid: no fluid or effusion accumulation unless distention is due to a disease that causes fluid buildup.
\item Location: can affect any part of the chest, including the heart, lungs, or diaphragm.
\item Opacity: normal or slightly more opaque, depending on the cause of the distention.
\item Other: increased size of certain structures; displacement of structures; overall crowded appearance.
\item Patterns: no specific patterns, but there may be displacement of structures.
\item Shape: enlargement of certain structures, such as the heart, lungs or diaphragm.
\item Texture: smooth or uniform, but the overall lung field may appear crowded or compressed.
\end{itemize}\\
\midrule
Shift & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: no specific border changes related to shift.
\item Fluid: may be present, particularly if the shift is due to a large pleural effusion (fluid around the lung) or pneumothorax (air in the chest outside the lung).
\item Location: a shift usually refers to the movement of the mediastinal structures away from their usual central position and could be towards any part of the chest.
\item Opacity: no specific opacity changes related to shift.
\item Others: the diaphragm, which should be a mirror image on both sides, may also appear displaced or elevated on the side of the shift. there may also be evidence of lung collapse or atelectasis on the side opposite to the shift.
\item Patterns: asymmetry between the two sides of the chest, with the mediastinal structures appearing closer to one lung than the other.
\item Shape: the mediastinal structures (heart, trachea, major vessels) may appear shifted or off-center.
\item Texture: no specific texture changes related to shift.
\end{itemize}\\
\midrule
Stent & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: sharp and clear, distinctly separating the stent from the surrounding tissue.
\item Fluid: no fluid accumulation or effusion.
\item Location: usually located in the region of the heart or major blood vessels.
\item Opacity: more opaque and less transparent, appearing as a bright white line or tube.
\item Other: symmetric appearance, contrast between the bright stent and the darker surrounding tissues, clear visibility of the stent's entrance and exit points.
\item Patterns: no specific patterns, just a distinct, linear structure that stands out against the darker background.
\item Shape: clear and defined shape, often straight or slightly curved, resembling a small pipe or tube.
\item Texture: smooth and uniform, with no variations or irregularities.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel16}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Pressure & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: normal or distorted depending on the cause.
\item Fluid: possible fluid accumulation or effusion if the pressure is caused by a mass or tumor.
\item Location: may affect any part of the chest, depending on the source of pressure.
\item Opacity: depending on the cause, can vary from normal to more opaque or transparent. for instance, lung collapse due to pressure would appear more opaque.
\item Other: displacement of structures, such as the heart or trachea; possible rib deformities or fractures if pressure is due to trauma.
\item Patterns: no specific patterns, changes would be related to the cause of pressure.
\item Shape: abnormalities such as a shift in the position of the mediastinum or diaphragm, or changes in the size and shape of the lungs.
\item Texture: usually normal unless there is a lung collapse or fluid accumulation.
\end{itemize}\\
\midrule
Lesion & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: may have a well-defined border, or it could be fuzzy and unclear.
\item Fluid: absence or presence of fluid can indicate different types of lesions.
\item Location: can appear anywhere in the lung.
\item Opacity: more opaque and less transparent, appearing whiter or darker compared to the surrounding lung tissue.
\item Other: size can vary, calcification may be present in some lesions, and if the lesion is growing, it can cause a shift in surrounding structures.
\item Patterns: solitary or multiple depending on the type of lesion.
\item Shape: could be a round, oval, or irregular spot, often with a clear, sharp edge.
\item Texture: solid or hollow, depending on the type of lesion.
\end{itemize}\\
\midrule
Finding & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: borders that are blurred, irregular, or abnormally sharp could indicate a disease or condition.
\item Fluid: fluid accumulation or effusion with a cloudy appearance could indicate an issue.
\item Location: note if the finding is in an unusual location or if there is asymmetric appearance between two sides of the chest.
\item Opacity: this will depend on the finding, but generally, anything that appears unusually dark or light could be significant.
\item Other: any other findings that seem out of the ordinary, such as unexplained shadows, lines, or spots, could be significant. increased or decreased lung volume could also be indicative of a condition or disease.
\item Patterns: unusual patterns, such as spots, streaks, or clusters, could be significant.
\item Shape: look for any structures that appear misshapen, distorted, or out of place.
\item Texture: any areas that appear grainy, mottled, patchy, or have a different texture from the surrounding tissue could indicate a problem.
\end{itemize}\\
\midrule
Borderline & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: clear and distinct from the surrounding lung tissue.
\item Fluid: no fluid accumulation or effusion is usually visible in this condition.
\item Location: centered in the chest, between the lungs.
\item Opacity: the heart area appears white and opaque compared to surrounding tissue.
\item Other: the heart occupies more than half of the chest's width, but not significantly larger; the lung fields will appear normal, without opacity or fluid accumulation; there may be displacement of the surrounding structures due to the increased heart size.
\item Patterns: consistent and symmetrical on both sides.
\item Shape: the heart silhouette is round or oval, but larger than normal.
\item Texture: smooth, consistent, and homogeneous texture.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel17}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Hardware & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: very clear, sharp edges, unlike the blurry or fuzzy edges of lung or other soft tissue.
\item Fluid: not typically associated with fluid accumulation, but could be surrounded by fluid if there's a complication.
\item Location: can be anywhere, depending on the type of hardware, but most commonly seen in the chest wall, spine, surrounding the heart, or within the lungs.
\item Opacity: very opaque, appearing as bright white objects.
\item Other: casting of shadows, presence of surgical clips, wires, or sutures.
\item Patterns: often geometrical, may resemble known objects, such as the shape of screws, plates, valves, wires, tubes, or pacemakers.
\item Shape: the shape of the hardware can be very different, but it is often linear or geometric.
\item Texture: smooth and well-defined, unlike the softer textures in lung tissue.
\end{itemize}\\
\midrule
Dilation & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the borders of the dilated structures are well-defined and may appear thicker or more prominent.
\item Fluid: no fluid or effusion accumulation typically associated with dilation.
\item Location: the location of dilation can vary, but it is usually visible in the area of the bronchial tubes.
\item Opacity: the area of dilation may be more transparent or darker due to the increased air content.
\item Other: increased lung volume, visible air-filled spaces, and distortion of nearby structures.
\item Patterns: no specific patterns, but the affected structure may show a tubular or cylindrical pattern due to dilation.
\item Shape: an enlarged and distorted shape of the bronchial tubes or other structures.
\item Texture: the texture inside the dilated area might appear smooth due to increased air content.
\end{itemize}\\
\midrule
Congestive heart failure & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: the outline of the heart may appear fuzzy or blurred.
\item Fluid: fluid accumulation or effusion in the lung fields and around the heart.
\item Location: the heart, located in the center of the chest, is the main organ affected.
\item Opacity: more opaque, appearing as white or cloudy around the heart region.
\item Other: widening of the vascular markings, particularly in the upper lung fields; presence of pleural effusion (fluid in the space between the lungs and chest wall); increased lung volume.
\item Patterns: fluid accumulation may appear in a butterfly or bat-wing pattern in the lungs.
\item Shape: heart appears enlarged and rounder than normal.
\item Texture: grainy texture in the lung fields due to fluid accumulation.
\end{itemize}\\
\midrule
Redistribution & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: no specific border, normal lung fields.
\item Fluid: no fluid or effusion accumulation unless there's a concurrent condition.
\item Location: vessels in the upper part of the lungs appear larger and more numerous than usual.
\item Opacity: normal or slightly more opaque, depending on the underlying cause.
\item Other: heart size may appear larger, especially if the redistribution is due to heart failure.
\item Patterns: appearance of more blood vessels in the upper part of the lungs and fewer in the lower part.
\item Shape: no specific shape, it's more about the redistribution of blood vessels.
\item Texture: no specific texture, normal lung fields.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel18}
\end{table*}
}{\footnotesize\begin{table*}[t]

\centering
\begin{tabular}{|l|p{14cm}|}
\toprule
\textbf{Findings} & \textbf{Aspect Descriptions} \\
\midrule
Aspiration & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: unclear or fuzzy, blending into the surrounding lung tissue.
\item Fluid: possible fluid accumulation, appearing as a dense, cloudy area.
\item Location: usually in the right lower lobe of the lung, but can be in any part depending on the position of the patient when aspiration occurred.
\item Opacity: more opaque, appearing denser or whiter than the surrounding lung tissue.
\item Other: presence of a foreign body or object; collapsed lung tissue around the aspirated material; and possible widened mediastinum if the aspirated material is in the central airways.
\item Patterns: dense patch or cloud that is not uniformly spread out.
\item Shape: irregular, with no specific shape, appearing as a patch or cloud in the lung.
\item Texture: appears grainy or fluffy, similar to a hazy cloud.
\end{itemize}\\
\midrule
Abnormal observation & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: borders might be fuzzy, blurred, or sharp depending on the nature of the disease.
\item Fluid: fluid accumulation or effusion may or may not be present.
\item Location: can occur anywhere within the chest, including in the lungs, heart, or bones of the chest wall.
\item Opacity: may vary widely depending on the specific disease, but often includes abnormal white or dark spots.
\item Others: abnormalities in the size or shape of the heart, unusual bone structures, or any other unusual features not typically seen in a healthy chest x-ray.
\item Patterns: patterns can vary widely, but any unusual or asymmetric pattern might be indicative of a rare disease.
\item Shape: irregular shapes, nodules, or masses that do not normally appear in the lungs.
\item Texture: could be grainy, mottled, or dense depending on the disease.
\end{itemize}\\
\midrule
% Excluded_obs & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
% \item Border: unspecified.
% \item Fluid: may have fluid accumulation.
% \item Location: breastbone or heart or any other locations.
% \item Opacity: can be more or less opaque.
% \item Others: presence of surgical hardware, changes in organ size or position, the presence of foreign bodies or grafts.
% \item Patterns: vary, lung collapse or solidification of lung tissue.
% \item Shape: irregular, round, oval, or have unique shapes based on the context.
% \item Texture: smooth, grainy, mottled, or contains specific features.
% \end{itemize}\\
% \midrule
Covid19 & \vspace{-0.8em}\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
\item Border: fuzzy or unclear, blending into the surrounding lung tissue.
\item Fluid: no specific fluid accumulation or effusion.
\item Location: typically affects both lungs and often located at the lung's edges or periphery.
\item Opacity: bilateral and peripheral ground-glass opacities, appearing as hazy, gray areas in the lungs.
\item Other: "crazy-paving" pattern, which resembles irregularly placed paving stones. it's seen as a combination of ground-glass opacity and interlobular septal thickening. asymmetry between the two lungs is often observed.
\item Patterns: multifocal patchy consolidation, appearing as several cloudy areas that are not evenly spread.
\item Shape: irregular, round, patchy areas in the lung.
\item Texture: fluffy, grainy or frosted glass appearance within the lung area.
\end{itemize}\\
\midrule
\end{tabular}
\label{yourlabel19}
\end{table*}
}
